VTruST: Controllable value function based subset selection for Data-Centric Trustworthy AI

Trustworthy AI is crucial to the widespread adoption of AI in high-stakes applications with fairness, robustness, and accuracy being some of the key trustworthiness metrics. In this work, we propose a controllable framework for data-centric trustworthy AI (DCTAI)- VTruST, that allows users to control the trade-offs between the different trustworthiness metrics of the constructed training datasets. A key challenge in implementing an efficient DCTAI framework is to design an online value-function-based training data subset selection algorithm. We pose the training data valuation and subset selection problem as an online sparse approximation formulation. We propose a novel online version of the Orthogonal Matching Pursuit (OMP) algorithm for solving this problem. Experimental results show that VTruST outperforms the state-of-the-art baselines on social, image, and scientific datasets. We also show that the data values generated by VTruST can provide effective data-centric explanations for different trustworthiness metrics.

==> intro_old.tex <==
\section{Introduction}

% \tr{
% Trusted-AI \cite{} or Resposible AI \cite{} is an important resquirement for modern AI systems.\\
% Data-centric approches to AI has certain advantages:\\
% - Explainability in terms of data-points.
% - Efficiency in terms of being able to use a minimal set of essential datapoints for training.\\
% - Inherennt measures of Data-quality for the end task using data valuation.\\
% controllable framework for the composition of multiple value functions.\\
% Many data valuation and subset selection methods have been developed. While these methods are general, it is not clear whether a single framework can be used for trading off between multiple efficiency, robustness and fariness value functions.\\
% We demonstrate that a single Data-centric approach can be used to achieve state-of-the-art performance for all the above tasks. \\
% We also propose a sampling scheme for data augmentation for multiple corruptions which leads to an initial small training dataset, which further leads to efficient DCAI approach to robustness.\\
% }

% Data centric approach along with the proposed algorithm leading to trustworthy AI.

% Can there be a purely data centric approach for robustness and fairness? Purely data centric approach - allowed to only augment and select data.

The field of artificial intelligence (AI) has seen rapid advancements leading to its involvement in our daily lives. 
%This usefulness comes with heightened responsibility especially in high-stake applications such as predicting the risk of criminal recidivism \citep{Angwin2016Machine}, autonomous driving \citep{kohli2020enabling,chen2021deep}, disaster management \citep{linardos2022machine} and many more.
% Starting from predicting shares in stock markets \citep{}, to convicting a person of crime \citep{}, or analysing medical reports based on images \citep{}, and notably, using ChatGPT as educational tool \citep{}, AI has become an integral part of our daily life. This leads to a rising societal awareness for the systems to be trustworthy \citep{} or responsible \citep{}. 
In order for users to trust the decision of the AI algorithms, it is essential for them to be fair, reliable and robust under different circumstances. 
%These algorithms work with both data and models as their integral components.
% Traditionally there are two popular paradigms in AI - \textit{model-centric AI} and \textit{data-centric AI}. In model-centric AI, the researchers try to improve the model by keeping the data fixed so that they perform better on the downstream tasks. On the other hand, in data-centric AI, the data is systematically engineered to fix the AI systems.
There is a substantial body of research in the area of model-centric AI where the need for making the models robust \citep{wang2022removing, 9892068} or fair \citep{roh2020fairbatch, romano2020achieving} or unbiased \citep{gat2020removing, majumdar2021attention} or explainable \citep{pillai2021explainable,sarkar2022framework} has been explored while keeping the data fixed. However, the core input to the models, \textit{the data}, has undergone reasonably less exploration. 
%While there has been a lot of research surrounding developing models that are robust \citep{wang2021augmax,shi2021fast} or fair \citep{nabi2022optimal,romano2020achieving}, the aspect of extracting robust or fair datapoints \citep{roh2021sample} has been less explored.
% For several decades, the focus was on using models on large datasets without comprehending its fidelity to the underlying problem.
With the upcoming progress in the field of \textit{Data-Centric AI} %\footnote{\url{https://datacentricai.org/}} 
\citep{hajij2021data,motamedi2021data}, currently the focus has shifted to creating quality datasets to avoid data cascades in real world setting.
%\footnote{\url{https://ai.googleblog.com/2021/06/data-cascades-in-machine-learning.html}}. 
%The DCAI approach comes with several advantages - identifying data points that explain certain model characteristics \citep{seedat2022data,ethayarajh2022understanding}, selecting useful datapoints for efficient training \citep{das2021tmcoss,pmlr-v162-pooladzandi22a}, discarding noisy samples deviating training trajectory \citep{NEURIPS2020_e6385d39,das2021finding}, scoring datapoints based on a value function reflecting their contribution to the task \citep{yoon2020data,lin2022measuring} and many more. 
%establishing consensus with crowdsourced annotations \citep{wang2021human,9069472} and many more. 
%The effectiveness of the AI system is assessed on the basis of both model and the data interlinked with the model.

In this work, we design a data-centric approach to achieving trustworthy AI through a controllable data valuation framework with the composition of several value functions aimed at key trustworthy AI metrics - fairness, robustness, and explainability. 
% We formulate the value functions targeted specifically toward the trustworthy goals and then incorporate them into our proposed framework. 
Additionally, we allow the users to control the balance between the trustworthiness metrics.
% Not clear why/what exactly the framing of the problem is - the following dives too deep into details without context -- PLS CHECK
We pose the problem of training data valuation and selection as an online sparse approximation problem, which we execute using a novel online version of OMP \citep{5895106}. 
Unlike in OMP where the decision of including the optimal variables happens iteratively \textit{looking at the entire data each time}, our proposed method, VTruST, works in an online setup where the data arrives incrementally and the decision of inclusion/exclusion happens on the fly by \textit{only iterating over the already included variables}. 
We add a \textit{DataReplace} component which enforces conditions based on the projections leading to the replacement of already selected non-optimal features. 
% The following text seems to have been partly repeated earlier and in related work below - PLS CHECK
% While there has been a lot of research surrounding developing models that are robust \citep{wang2021augmax,shi2021fast} or fair \citep{nabi2022optimal,romano2020achieving}, the aspect of extracting robust or fair datapoints \citep{roh2021sample} has been less explored.
% Likewise, the areas of data valuation using value functions or subset selection have also gained much traction.  
To the best of our knowledge, this is one of the first works to provide a single unified framework for balancing between the multiple value functions, followed by data valuation and extraction of subsets. These subsets when trained from scratch, lead to fairer, more robust, or more accurate models depending on the usage of value functions. 

To summarize, our main contributions in the paper are:
% \begin{enumerate}
    (1) We design a data-centric controllable selection framework that helps us obtain a subset of training datapoints specifically suited for trustworthiness metrics.
    (2) We formulate the value functions for the metrics of fairness, robustness, and accuracy. We also design a sampling algorithm for constructing augmented datasets for robustness.
    %(3) We provide theoretical derivations of the conditions used in VTruST and show that they are sufficient for the exact recovery of the sparse solution.
    (3) We demonstrate that VTruST with subsets of even 40\% of the original dataset, is able to outperform all state-of-the-art baselines by $\sim 10-20\%$ and can also provide data-centric explanations behind its performance.
    
    % tasks of achieving fairness on benchmark datasets like COMPAS, Adult Census, as well as attain robustness on image classification tasks using standard CIFAR-10-C, MNIST-C and Tiny ImageNet-C datasets.
% \end{enumerate}
% Besides formulating the value functions aimed at the goals of trustworthy AI, we also propose a sampling algorithm for constructing augmented datasets for the task of robustness. We demonstrate that our data-centric approach with subsets of upto even 20\% of the original dataset, is able to outperform all state-of-the-art baselines by $\sim 10-20\%$ in the tasks of achieving fairness on benchmark datasets like COMPAS, Adult Census, as well as attain robustness on image classification tasks using standard CIFAR-10-C, MNIST-C and Tiny ImageNet-C datasets.

==> proof.tex <==
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}

% \subsection{Conditions for Optimality of the Selected Subset}
% \label{sec:conditions}

\textbf{Conditions for Optimality of the Selected Subset}:
Considering the proposed algorithm is an online sparse approximation problem, the optimality shall depend on the order in which the features of the training datapoints arrive. We want to derive the conditions for an ordering $\Pi(\vec{X})$ of columns of $\vec{X}$ to produce a correct combination of optimal features $\vec{X}_{(T)}$, where $\vec{X}$ is the set of all features $\{\vec{X}_1,..,\vec{X}_N\}$ and $\vec{X}_{(T)}$ is the optimal/correct set of features approximating the value function $\vec{y}$.
% Let $\mathcal{X}$ be the set of all $k$-sparse approximations of output $\vec{y}$ from $\vec{X}$ , i.e $\forall \vec{X}_{(T)} \in \mathcal{X}$ such that, (i) $|\vec{X}_{(T)}| \leq k$ and (ii) $\vec{y} - \beta^* \vec{X}_{(T)} = \vec{0}$ where $\beta^*$ is the optimal parameter and $\vec{X}_{(T)}$ is the optimal/correct set of features approximating the value function $\vec{y}$.

For the clarity of the proof, we consider a set of features outside the optimal set $\vec{X}_{(T)}$ denoted by $\vec{X}_{(O)}$. We index the features of selected datapoints by $\vec{X}_{(s_m)}$  where $m \in \{1,2,..,N\}$. Using $\vec{X}_{(T)}$, we can obtain the set of optimal selected features as $\vec{X}_{(c_m)} : \vec{X}_{(s_m)} \cap \vec{X}_{(T)}$ ; and the non-optimal ones as $\vec{X}_{(o_m)} : \vec{X}_{(s_m)} \setminus \vec{X}_{(c_m)}$. The algorithm aims to reduce the residual $\vec{\rho}_m$ which as we know is  $\vec{\rho}_m = \vec{y} - \vec{\beta}_{(s_m)}\vec{X}_{(s_m)}$. Using the above, we can also rewrite it as $\vec{\rho}_m : \vec{y} - \vec{\beta}_{(c_m)} \vec{X}_{(c_m)}  - \vec{\beta}_{(o_m)} \vec{X}_{(o_m)} $. We define the theorem which states the conditions for selection of an optimal set of elements.

% In order to derive the conditions, we further define some additional notations. Starting from $\vec{X} = \{\vec{X}_1,..,\vec{X}_N\}$, which defines the features of all training datapoints, we define $\vec{X}_{(T)}$ as the optimal/correct set of features approximating the value function $\vec{y}$ where $T = \{i : \beta_i \neq 0\}$ ; $\vec{X}_{(O)} : \vec{X} \setminus \vec{X}_{(T)} $ as the features outside the optimal set ; $\vec{X}_{(s_m)}$ as the set of features of selected datapoints till timestep $m$ where $m \in \{1,2,..,N\}$ ; $\vec{X}_{(c_m)} : \vec{X}_{(s_m)} \cap \vec{X}_{(T)}$ as the set of optimal/correct set of selected features; $\vec{X}_{(o_m)} : \vec{X}_{(s_m)} \setminus \vec{X}_{(c_m)}$ as the set of features outside the optimal set and $\vec{\rho}_m : \vec{y} - \vec{X}_{(s_m)} \vec{\beta}_{(s_m)}$ as the residual vector which can also be written in the form of  $\vec{\rho}_m : \vec{y} - \vec{\beta}_{(c_m)} \vec{X}_{(c_m)}  - \vec{\beta}_{(o_m)} \vec{X}_{(o_m)} $.



% \begin{itemize}
%     \item $|\vec{X}_{(T)}| \leq k$
%     \item $\vec{y} - \beta^* \vec{X}_{(T)} = \vec{0}$ where $\beta^*$ is the optimal parameter.
% \end{itemize}

% We want to derive the conditions for an ordering $\Pi(\vec{X})$ of columns of $\vec{X}$ to produce a correct combination of optimal features.

\footnotesize
\begin{theorem}[Conditions in terms of Algorithm]
\label{theorem1}
$\forall m \in \{k+1, \dots N\} \mbox{ } \exists \vec{X}_{(T)} \in \mathcal{X} \mbox{ } s.t. \mbox{ } \forall x \in \vec{X}_{(T)} \mbox{ }, \mbox{ }\forall z \in \vec{X}_{(o_m)}$ if $|\vec{\rho}_m^Tx| > |\vec{\rho}_m^Tz|$ and $\beta_z < 0$ ,  then $x$ will be included in $\vec{X}_{(s_{m+1})}$ by replacing $z$ that satisfies the condition $max_z |\vec{\rho}_m^Tz| + \beta_z$
\label{theo:1}
\end{theorem}
\normalsize
The proof is provided in the Appendix.

% \newcommand{\qed}{\hfill\blacksquare}
% $\qed$


